Schema-agnostic Progressive Entity Resolution (extended version)

Entity Resolution (ER) is the task of finding entity profiles that correspond to the same real-world entity. Progressive ER aims to efficiently resolve large datasets when limited time and/or computational resources are available. In practice, its goal is to provide the best possible partial solution by approximating the optimal comparison order of the entity profiles. So far, Progressive ER has only been examined in the context of structured (relational) data sources, as the existing methods rely on schema knowledge to save unnecessary comparisons: they restrict their search space to similar entities with the help of schema-based blocking keys (i.e., signatures that represent the entity profiles). As a result, these solutions are not applicable in Big Data integration applications, which involve large and heterogeneous datasets, such as relational and RDF databases, JSON files, Web corpus etc. To cover this gap, we propose a family of schema-agnostic Progressive ER methods, which do not require schema information, thus applying to heterogeneous data sources of any schema variety. First, we introduce two naive schema-agnostic methods, showing that straightforward solutions exhibit a poor performance that does not scale well to large volumes of data. Then, we propose four different advanced methods. Through an extensive experimental evaluation over 7 real-world, established datasets, we show that all the advanced methods outperform to a significant extent both the na\"ive and the state-of-the-art schema-based ones. We also investigate the relative performance of the advanced methods, providing guidelines on the method selection.

==> section/exp_fig.tex <==
\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.92\textwidth]{images/exp/large_10}
	%\vspace{-13pt}
	\caption{Recall progressiveness on
	\textsf{heterogeneous} datasets.}
	%\vspace{-8pt}
	\label{fig:large}
\end{figure*} 

\begin{figure}[ht!]
	\centering
	\includegraphics[width=0.47\textwidth]{images/exp/auc_large}
	%\vspace{-10pt}
	\caption{AUC.}
	%\vspace{-15pt}
	\label{fig:auc_large}
\end{figure}

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.93\textwidth]{images/exp/time}
	\vspace{-10pt}
	\caption{Time experiments with (a) \textsf{mf1:edit-dist}, and (b) \textsf{mf:jaccard-sim}; (c) initialization times.
	}
	\vspace{-14pt}
	\label{fig:time}
\end{figure*} 

==> section/experiments__old.tex <==
\section{Experiments}
\label{sec:experiments}


\input{tables/datasets}

\noindent
\textbf{System setup}.
All experiments have been performed on a server running Ubuntu 14.04, with 80GB RAM, and an Intel
Xeon E5-2670v2 2.50GHz CPU. All the methods are implemented in Java 8, and
the code is publicly available\footnote{\url{https://stravanni.github.io/progressiveER/}}.

\vspace{2pt}
\noindent
\textbf{Datasets.}
For the experimental evaluation, we employ 7 diverse real-world datasets that are widely
adopted in the literature as benchmark data for \textsf{ER} \cite{DBLP:journals/tkde/Christen12, DBLP:journals/pvldb/KopckeTR10, DBLP:journals/tkde/PapadakisKPN14, DBLP:journals/pvldb/0001SGP16, DBLP:journals/pvldb/SimoniniBJ16, btc-2009}.
Their characteristics are reported in Table \ref{table:datasets}.
We distinguis
Three of them (\texttt{census}, \texttt{restaurant},
\texttt{cora}, and \texttt{cddb}) are extracted from a single data source
containing duplicated profiles, hence meant to test \textsf{Dirty ER} tasks.
The remaining datasets (\texttt{movies}, \texttt{dbpedia}, and \texttt{freebase}) are suitable for testing \textsf{Clean-clean ER}, as they are extracted from two different data sources, where matching profiles exist only between a source and another:
%\texttt{articles} from \texttt{dblp.org} and \texttt{dl.acm.org};
%\texttt{products} from \texttt{Abt.com} and \texttt{Buy.com};
\texttt{movies} from \texttt{imdb.com} and \texttt{dbpedia.org};
\texttt{dbpedia} from two different snapshots of DBpedia (\texttt{dbpedia.org} 2007-2009) --- due to the constant changes in DBpedia, the two versions share only 25\% of the \textit{name-value} pairs, forming an non-trivial \textsf{ER} task \cite{DBLP:journals/tkde/PapadakisKPN14,DBLP:journals/tkde/PapadakisIPNN13};
\texttt{freebase} from \texttt{developers.google.com/freebase/} and \texttt{dbpedia.org} (extracted from \cite{btc-2009}).
% , hence meant to test \textsf{Clean-clean ER}
% tasks.
For all the datasets the ground truth is known.

\vspace{2pt}
\noindent
% \subsubsection{Metrics}
\textbf{Metrics.}
To evaluate the effectiveness of a \textsf{Batch ER} method $m$ over a profile
collection $P$, we use \textsf{recall}, which measures the portion of
detected matches: $recall = |\mathcal{D}_m|/|\mathcal{D}_P|$,
where $\mathcal{D}_m$ denotes the set of matches detected (emitted) by $m$,
while $\mathcal{D}_P$ stands for the set of all matches in $P$.

In \textsf{Progressive ER}, we are interested in how fast matches are
emitted. To illustrate this, we consider \textsf{recall progressiveness} by
plotting the evolution of recall (vertical axis) with respect to the
\textit{normalized number of emitted comparisons} (horizontal axis): $ec^*{=}ec/|\mathcal{D}_P|$,
where $ec$ is the number of emitted comparisons at a certain time during the
processing. The purpose of this normalization is twofold: \emph{(i)} it allows
the use of the same scale among different datasets, and \emph{(ii)} it
facilitates the comparison of the methods to the \textit{ideal} one,
which achieves recall=1 after emitting just the first $|\mathcal{D}_P|$
comparisons, i.e., at $ec^*{=}1$.

% To assess the \textit{recall progressiveness} of a method, i.e., how fast existing matches are emitted, we express the recall in function of the 
To facilitate the comparisons between progressive methods, we quantify their
progressive recall using the \textit{area under the curve} (AUC) of the
above plot.\footnote{The AUC expressed in function of $ec$ (not the normalized
$ec^*$) is known in the literature as \textit{progressive recall}
\cite{DBLP:journals/pvldb/FirmaniSS16}, and is employed for the same purpose.}.
%We measure of the recall expressed in function of $nc^*$ to assess the quality
% of a progressive method
For a method $m$, we indicate with $AUC_m@ec^*$ the value of AUC for a given
$ec^*$; for instance, $AUC_{PSN}@5$ is the area under the recall curve of the
method \textsf{PSN} after the emission of $ec{=}5{\cdot}|\mathcal{D}_P|$ comparisons.
%In particular, we measure the $AUC_m@nc^*$.
To restrict $AUC_m@ec^*$ to the interval $[0,1]$, we normalize it with the
performance of the ideal method: $AUC_m^*@ec^* =
\frac{AUC_m@ec^*}{AUC_{ideal}@ec^*}$. 
$\mathbf{AUC_m^*@ec^*}$ is called \textsf{normalized area under the curve}:
% \begin{equation*}
% \end{equation*}
% where \textit{ideal} indicates the \textit{ideal} method.
% Hence, $AUC_m^*$ is in the interval (0,1], where 
higher values correspond to a better \textit{progressiveness}, with the ideal
method having $AUC_{ideal}^*{=}1$ for any value of $ec^*$.

For the time performance evaluation of a method $m$, we consider the \textit{initialization time} and the \textit{comparison time}:
the former is the time required to emit the first comparison, considering all the pre-processing steps (e.g., Token Blocking, Block Purging, Block Filtering for Blocking Graph-based methods);
the latter is the average time between two consecutive comparison emissions.
%We call \textbf{initialization overhead} the time required for the initialization phase (i.e., the time between receiving the input data and producing the first comparison), while \textbf{emission overhead} is the average time required for returning each comparison.

%Notice that, in the time experiments of Section \ref{sec:results}, 
%It is important to stress that our proposed measure for the \textit{recall progressiveness} is decoupled from the \textit{matching function} actually employed when performing the complete \textsf{ER} process, as discussed in Section \ref{}.

\vspace{2pt}
\noindent
% \subsubsection{Baselines}
% \label{sec:baseline}
\textbf{Baselines.}
%Our baselines are \textsf{PSN}, which is the current state-of-the-art method for \textsf{Progressive ER} \cite{DBLP:journals/tkde/PapenbrockHN15,DBLP:journals/tkde/WhangMG13}, and \textsf{SA-PSN}.
As baseline methods, we use \textsf{PSN}, \textsf{SA-PSN}, and
\textsf{SA-PSAB}. For the \textsf{Dirty ER} datasets, the best blocking keys for
\textsf{PSN} are known from \cite{DBLP:journals/tkde/Christen12}.
For the \textsf{Clean-clean ER} datasets, though, we do not know the best
blocking keys. Thus, we consider only \textsf{SA-PSN} and
\textsf{SA-PSAB} as baselines.
%The \textsf{PSN} \textit{dynamic} variant proposed in \cite{DBLP:journals/tkde/PapenbrockHN15} in a \textit{static} setting, i.e., without exploiting the feedback of the resolution function, is equivalent to \cite{DBLP:journals/tkde/WhangMG13} (see Section \ref{} \note{if we discuss this before}).

%It is important to notice that the blocking key selection is typically a time consuming pre-processing step \cite{}.
%Moreover, if more than one source is involved (i.e., in \textsf{Clean-Clean ER}), additional time has to be spent to perform the schema alignment before the key selection.
%In the time experiments of Section \ref{} we are not considering thee additional overhead time, which are not required to perform our methods.
%Nevertheless, our schema-agnostic methods outperforms schema-based ones on as well.

%As discussed in Section \ref{sec:naiveSolutions}, we also implemented \textsf{SA-PSA},
%but it showed a recall progressiveness and an execution time significantly worse than all the other methods, hence we left it out from the experimental evaluation.
%\note{(If we leave it out, otherwise we change this paragraph.)}

% \subsubsection{Configuration}


% \medskip
\vspace{2pt}
\noindent
\textbf{Parameter configuration}. We apply the following settings to all
datasets: for \textsf{SA-PSAB}, we set $l_{min}$=2.
For \textsf{LS-PSN} and \textsf{GS-PSN}, we set $w_{max}$=20 for structured datasets and $w_{max}$=200 for large and heterogeneous datasets.
For the methods of Section \ref{sec:bg-methods}, we use the \textit{Token Blocking workflow} to derive the redundancy-positive block collection.
This workflow has been experimentally verified to address effectively and efficiently the Volume and Variety of Web data \cite{DBLP:conf/edbt/0001PPK16}. It consists of the following steps: \emph{(1)} Schema-agnostic Standard Blocking \cite{DBLP:journals/pvldb/0001APK15}, a.k.a. Token Blocking, creates a separate
block for every attribute value token that stems from at least two profiles.
\emph{(2)} \textit{Block Purging} \cite{DBLP:journals/tkde/PapadakisIPNN13} discards large blocks that correspond to stop words, involving more than 10\% of the input profiles.
\emph{(3)} \textit{Block Filtering} \cite{DBLP:conf/edbt/0001PPK16} retains every profile in 80\% of its most important (i.e., smallest) blocks. \emph{(4)} \textsf{ARCS}  performs edge weighting on the Blocking Graph. Finally, for \textsf{PPS}, we set $\alpha = 10$, since preliminary experiments verified that it yields good performance.

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.9\textwidth]{images/exp/large_10}
	%\includegraphics[width=0.8\textwidth]{images/exp/large_v_20}
	%\vspace{-13pt}
	\vspace{-8pt}
	\caption{Recall progressiveness on \textsf{large} and \textsf{heterogeneous} datasets.}
	%\vspace{-8pt}
	\label{fig:large}
\end{figure*} 


\begin{figure}[t!]\centering
	\includegraphics[width=0.4\textwidth]{images/exp/auc_large}
	%\includegraphics[width=0.47\textwidth]{images/exp/auc_large_50}
	\vspace{-8pt}
	\caption{AUC (on \textsf{large} and \textsf{heterogeneous} datasets).}
	\vspace{-5pt}
	\label{fig:auc_large}
\end{figure}


% For all methods, we use the \textsf{ARCS} 
% weighting scheme to associate every comparison with a score in $[0,1]$ that is
% analogous to the likelihood that the corresponding profiles are matching (note
% that normalization is needed). Numerous experiments have
% verified that \textsf{ARCS} consistently achieves a good balance between
% effectiveness and efficiency over a series of datasets
% \cite{DBLP:conf/edbt/0001PPK16}; this applies to both \textsf{Clean-clean} and
% \textsf{Dirty ER}. Note also that \textsf{ARCS} is schema-agnostic, tackling
% inherently the Variety of Web data.

% $\bullet$ For \textsf{GS-PSN} , the \textit{maximum window} is 20 on all the
% datasets.
% $\bullet$ For all the \textsf{BG}-methods, the basic block collection is
% generated by employing the workflow configuration described in Section \ref{sec:bg-methods}.
% $\bullet$ For \textsf{NC-CEP}, on all the datasets, we employ the following
% heuristic: $k{=}10{\cdot}\bar{k}$, which has experimentally shown to yield good performances.
% The same formula is employed in \textsf{CEP-pList}, for the emission of the comparisons of each profile.

%We use the following configurations:
%Here, we list the parameters configuration.
%For the sake of presentation, we report the result distinguishing between \textsf{SN}-methods and \textsf{BG}-derived; which are respectively derived from \textsf{SN}, (i.e., \textsf{PSN}, \textsf{SA-PSN}, \textsf{GS-PSN}, \textsf{LS-PSN}) and from \textsf{BG} (i.e., \textsf{CEP}, \textsf{NC-CEP}, \textsf{PBS}, \textsf{CEP-pList}).
%\noindent
%$\bullet$

%this value is generally sufficient to complete the \textsf{ER} for \textsf{PSN}, \textsf{SA-PSN}, and \textsf{LS-PSN}.
%\noindent
%$\bullet$
%As for the weighting schema for the blocking graph, we employ \textsf{ARCS}.
%Note that the other weighting schemas achieve similar performances in the experiments, and for the sake of the presentation, we do not report them here.
%\noindent
%$\bullet$
%For \textsf{CEP} we employ the \textit{memory driven} configuration.
%This configuration generates the higher overhead time for the initialization phase; nevertheless, we experimentally show in that it can be a valid method (Figure \ref{fig:time}).
%if the available memory is enough.
%\noindent
%$\bullet$

%The \textit{memory driven} configuration can achieves higher level of recall for some datasets, with a

% We derive the initial block collection from the \textsf{Token Blocking
% workflow}, which has been experimentally verified to address effectively and
% efficiently the Volume and Variety of Web data, while yielding
% redundancy-positive blocks \cite{DBLP:conf/edbt/0001PPK16}. It consists of the
% following steps:
% 
% \noindent
% \emph{(1)} Schema-agnostic Standard Blocking
% \cite{DBLP:journals/pvldb/0001APK15}, a.k.a. Token Blocking, creates a
% separate block for every attribute value token that stems from at least two
% profiles.
% 
% \noindent 
% \emph{(2)} \textit{Block Purging}
% \cite{DBLP:journals/tkde/PapadakisIPNN13} discards large blocks that correspond
% to stop words, involving more than 10\% of the input profiles.
% 
% \noindent
% \emph{(3)} \textit{Block Filtering}
% \cite{DBLP:conf/edbt/0001PPK16} retains every profile in 80\% of its most
% important (i.e., smallest) blocks. 

% \vspace{2pt}
% \noindent
% \textbf{Weighting scheme.} For all methods, we use the \textsf{ARCS} 
% weighting scheme to associate every comparison with a score in $[0,1]$ that is
% analogous to the likelihood that the corresponding profiles are matching (note
% that normalization is needed). Numerous experiments have
% verified that \textsf{ARCS} consistently achieves a good balance between
% effectiveness and efficiency over a series of datasets
% \cite{DBLP:conf/edbt/0001PPK16}; this applies to both \textsf{Clean-clean} and
% \textsf{Dirty ER}. Note also that \textsf{ARCS} is schema-agnostic, tackling
% inherently the Variety of Web data.

%  at \cite{}.
% \note{link to the code}


%For the \texttt{dirtyER} datasets best blocking key configuration for Sorted Neighborhood methods is known from related work \cite{}, so we for these dataset we consider both schema-based and schema-agnostic \textsf{PSN}.
%For \texttt{cleanCleanER datasets} we do not have blocking keys from other papers, so we just consider the schema-agnostic configuration.
%Notice that in this experiment our methods are \textbf{always} schema-agnostic.

% \subsection{Results}
% \label{sec:results}


\subsection{Effectiveness Evaluation on Large and Heterogeneous Dataset}

We first assess the relative effectiveness of
all methods with respect to recall progressiveness. The corresponding plots
appear in 
%  The goal of these experiments is to show the performance of our
% methods compared against the baselines.
%We perform for each method, on each dataset, both \textsf{Dirty ER} and \textsf{Clean-clean ER}.
% The results are shown in 
Figures \ref{fig:psn_d} and \ref{fig:pmb_d} for the \textsf{Dirty ER} datasets,
and in Figures \ref{fig:psn_c} and \ref{fig:pmb_c} for the \textsf{Clean-clean
ER} ones. The figures show the performance of all the methods up to $ec^*{=}10$,
i.e., they show the recall for a number of comparisons ten times the comparisons
required by the ideal method to complete each \textsf{ER} task.
%{\color{red}In each figure, at least one of the proposed methods reaches an highrecall (${>}80\%$) on all the datasets.\textbf{IS THIS TRUE?}}
%At the same time, they show the performance of all the methods in the early phase of their progressiveness.

The results confirm our intuition about the inefficiency of the na\"ive
schema-agnostic progressive methods, \textsf{SA-PSN} and \textsf{SA-PSAB},
since all advanced methods
% \textsf{SN}-methods and \textsf{BG}-methods 
outperform them to a significant extent
across all datasets. In fact, \textsf{SA-PSAB} is the worst performer, 
mainly due to the huge blocks in the highest layers of its suffix trees, which
entail too many useless comparisons. 

We stress the fact that our schema-agnostic methods also outperform the schema-based baseline (\textsf{PSN}) across all data\-sets.
The only dataset on which \textsf{PSN} performs well (and better than our Blocking Graph-based methods only) is \texttt{census} (see Figures~\ref{fig:psn_d}a and~\ref{fig:pmb_d}a).
%  dataset in
% with the only exception of 
This is because \texttt{census} contains very discriminative attributes, whose
values are employed as blocking keys for \textsf{PSN}\footnote{Encoded surnames
concatenated to initials and zipcodes.} and identify its duplicates with very high precision.
%\footnote{Please refer to \cite{DBLP:journals/tkde/Christen12} for the definition of the blocking keys for all the datasets.}
Moreover, the profiles of \texttt{census} have short strings as attribute
values:
% , i.e., every profile contains only a few tokens
%, with limited overlap
% most 
on average, every profile contains just 4-5 distinct tokens in its values.
Inevitably, this sparse information has significant impact on the performance of
Profile List- and Blocking Graph-based methods,
restricting the co-occurrence patterns that lie at their core, i.e., the
co-occurrences in windows for the former, and in blocks for the latter. 
The impact is larger in the latter case, due to the stricter definition of
co-occurrence, which requires the equality of tokens, not just their similarity.


% , and
% the average number of tokens per profile is 5.
% This is the worst case for \textsf{BG}-based methods, which rely on the token overlapping of the duplicates (see \textsf{BG}-methods on \texttt{census} in Figure \ref{fig:pmb_c}a).
% Remember that we are employing \textsf{Token Blocking} to build the starting block collection.
% Similar considerations can be made for \textsf{SN}-based methods in Figure \ref{fig:psn_d}a: they rely on the co-occurrence of the profiles on multiple windows to assign weights to the comparisons, hence, with a limited number of tokens, the co-occurrence in the windows is limited as well.

On the other hand, for datasets with a high token overlap of matching profiles, and low discriminative attributes, our methods significantly outperform the schema-based \textsf{PSN}.
For instance, in the \texttt{restaurant} dataset, the performance of
\textsf{R-CEP}, \textsf{NC-CEP}, and \textsf{CEP-pList} are very close to the ideal method (see Figure \ref{fig:pmb_d}b):
% In fact, their performance are very similar to the ideal: 
they reach recall${=}$1 for $ec^*$ close to 1, while for \textsf{PSN},
recall${=}$1\% at $ec^*{=}1$.

Among the Blocking Graph-based methods, \textsf{CEP-pList} is the best performer
for the \textsf{Clean-clean ER} datasets (Figure \ref{fig:pmb_c}).
For the \textsf{Dirty ER} ones, 
%though, there is no clear winner:
\textsf{NC-CEP} is the best performer over \texttt{cora} (Figure
\ref{fig:pmb_c}c), and \textsf{PBS} 
% is the best performer on 
over \texttt{census}
(Figure \ref{fig:pmb_d}a).
% , but on all the other \textsf{Dirty ER} datasets it is the worst performer.
%Similarly, there is no clear winner among 
Regarding 
the Profile List-based methods
% Among the \textsf{SN}-methods 
(Figures \ref{fig:psn_d} and \ref{fig:psn_c}), the best performers are \textsf{GS-PSN} with
\textsf{RCF} that is the best performer over \texttt{cora} (Figure
\ref{fig:psn_d}c), and \textsf{LS-PSN} with \textsf{RCF} over
\texttt{cddb} (Figure \ref{fig:psn_d}d). 
In the remaining datasets, their differences are insignificant. 
% there is not a clear winner.

%Finally, the results show that our methods outperform the schema-agnostic and schema-based baselines on all the  datasets; the only exception is the \texttt{census} dataset, where only our \textsf{SN}-methods has basically the same recall progressiveness of the schema-based baseline (\textsf{PSN}).

%We now discuss the $AUC_m^*$ of all the method to .
Hence, to understand which methods could be the best choice for a
given \textsf{ER} task, we now compare them with respect to their mean
value of normalized area under the curve.
% of $AUC_m^*$ for all 
% methods.
Figure~\ref{fig:auc} shows the mean $AUC_m^*$ of all methods across all 
datasets for four different values of $ec^*$: 1, 5, 10 and 20. 
% 
% for \textsf{Dirty-ER} and
% \textsf{Clean-clean ER} datasets respectively, the mean $AUC_m^*$ on all the datasets for different values of $nc^*$ is shown for all the methods.
%  
%  corresponds to high level of 
% The higher the value of $AUC_m^*$, the higher the recall reached by a method
% $m$.
In Figure~\ref{fig:auc}a, we observe that \textsf{LS-PSN} and \textsf{GS-PSN} in
combination with the \textsf{RCF} weighting scheme achieve the highest mean
$AUC_m^*$ over the \textsf{Dirty ER} datasets, across all values of $ec^*$.
Figure~\ref{fig:auc}b demonstrates that \textsf{CEP-pList} has the best
performance over the \textsf{Clean-clean ER} datasets for all the considered
values of $ec^*$. 
Note that
% Though, please notice that 
the performance of Blocking Graph-based methods has a higher variance than that
of Profile List-based methods in Figure~\ref{fig:auc}b, regardless of $ec^*$.
This is caused by the stricter definition of co-occurrence patterns they
employ (i.e., blocking key equality).
% due to the above considerations about the tokens
% overlap in the profiles.
%This is true for all the different values of $nc^*$ in Figure \ref{fic:auc_d} and Figure \ref{fig:auc}b

Overall, we conclude that if the profiles are represented by a large
number of tokens (${>}10$ in our experiments), the best performing method is
\textsf{CEP-pList}. Otherwise, in the presence of a limited number of tokens per profile, the
best choices are \textsf{GS-PSN} and/or \textsf{LS-PSN} with \textsf{RCF}.

% The choice between these two last methods can be driven by other factors, as for example their initialization time.

\subsection{Time Efficiency Evaluation.}

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.93\textwidth]{images/exp/time}
	\vspace{-10pt}
	\caption{Time experiments with (a) \textsf{mf1:edit-dist}, and (b) \textsf{mf:jaccard-sim}; (c) initialization times.
	}
	\vspace{-14pt}
	\label{fig:time}
\end{figure*} 

We note that our methods are general and decoupled from the matching function employed to determine whether two profiles are matching or not.
%\setlength{\skip\footins}{16pt}
%These functions are typically expensive, and generally requires labeled data and machine learning algorithms \cite{} \note{citation}.
To assess the benefit of our methods in terms of execution time though, we evaluate them in combination with two matching functions (\textsf{mf1:edit-distance} and \textsf{mf2:jaccard-sim}) based on the Damerau-Levenshtein edit distance \cite{DBLP:conf/acsw/Bard07} and the Jaccard similarity \cite{DBLP:books/cu/LeskovecRU14}, respectively\footnote{In a real-world scenario, each matching function would require a threshold parameter to discriminate between matching and non-matching pairs, on the basis of their edit distance (or Jaccard similarity).
Here, we are only interested in measuring the time performance, not the goodness of the matching function; hence, we do not employ any threshold, and the outcome of the matching function is assumed to be identical to the known ground truth.}. %between each profile paris emitted, considered as plain strings.
The former is meant to test the performance of our methods with an \textit{expensive} matching function, while the latter with a \textit{cheap} one.
The time complexities of \textsf{mf1:edit-distance} and \textsf{mf2:jaccard-sim} are $O(s{\cdot}t)$ and $O(s{+}t)$, respectively, where $s$ and $t$ are the lengths of the two strings to be compared (i.e., the two profiles compared with the matching function).
%In a real-world scenario, the edit distance is generally more powerful in detecting matching than Jaccard similarity.
%This is because the former considers the string at a character-level granularity and better capturing the distance between two tokens that differs only for a few characters;
%while the latter considers strings only at a token granularity, hence does not capture well the similarity of two tokens that differ only for a small portion of their characters.
%However,

%In a real-world scenario, each matching function would require a threshold parameter to discriminate between matching and non-matching pairs, on the basis of their edit distance (or Jaccard similarity).
%Here, we are only interested in measuring the time performance, not the goodness of the matching function; hence, we do not employ any threshold, and the outcome of the matching function is assumed to be identical to the known ground truth.

The schema-based methods are not considered in this evaluation, since they inherently require an additional overhead time to select the blocking keys, and (in the case of \textsf{Clean-clean ER}) to perform the schema-alignment.
%(required by the schema-based blocking keys).
There is a plethora of techniques to perform these two tasks \cite{DBLP:conf/icde/MelnikGR02,DBLP:journals/tkde/ShvaikoE13,DBLP:conf/aaai/MichelsonK06}.
It is out of the scope of this work to determine which is the best, since our proposed methods do not rely on them.
%Moreover, please notice that for \texttt{dbpedia} achieving a schema-alignment is challenging

In Figure~\ref{fig:time}, we report the result of the time experiments on the two largest datasets (\texttt{movies} and \texttt{dbpedia}), where the \textsf{ER} process is more time and resource consuming.
In particular, Figure~\ref{fig:time}a and Figure~\ref{fig:time}b plot the performance of all methods, considering both the initialization time, and the comparison time.
Here,  the comparison time includes both the emission time (i.e., the time to generate a comparison) and the time required for the execution of the matching functions.
The initialization times are listed in Figure~\ref{fig:time}c.
We note that for all methods and datasets the emission time is negligible (w.r.t. the time required by the matching functions): it is at least two orders of magnitude smaller than that required by the matching functions to compare two profiles.
Hence we do not report it here.

Overall, the results in Figure~\ref{fig:time} clearly show that our advanced methods produce most of the matches much earlier than the baseline, with both the expensive and cheap matching functions.
Profile List-based and Blocking Graph-based methods show different performance characteristics though.

The difference in the initialization times between each Profile List-based method and the baseline is negligible with both the matching functions (see the beginning of the x-axis of the bottom graphs in Figure~\ref{fig:time}a and Figure~\ref{fig:time}b); hence, they are able to outperform the baseline since the early stages of the process.
For Blocking Graph-based methods, the same consideration is valid only in the case where the expensive matching function is employed (see the beginning of the x-axis in Figure~\ref{fig:time}a top).
When the cheap matching function is employed, their initialization time may slightly affect the early stages of the process (Figure~\ref{fig:time}b top).
%This allow them to outperform the baseline during all the stages of the \textsf{ER} process.
%Differently, Blocking Graph-based methods involve the highest initialization time: when the expensive matching function is employed (Figure~\ref{fig:time}a) they outperform the baseline since the early stages of the process; while, when the cheap matching function is employed (Figure~\ref{fig:tile}b), their initialization time may affect the early stages of the process.
%For instance, \textsf{CEP-pList} in Figure~\ref{fig:time}b reaches a higher level of recall than \textsf{PSN} only for recall${>}$20\%.
Overall however, Blocking Graph-based methods achieve higher level of recall much earlier than Profile List-based methods.

%When employing \textsf{mf2:jaccard-sim} (refer to Figure~\ref{fig:time}b), a significantly cheaper matching function than \textsf{mf1:edit-distance}, the advantage of employing our %\textsf{BG}-method 
%Blocking Graph-based methods over the baseline is remarkable. {\bf ??? this is not true: I can see a very small difference between our methods in blue/green and the baseline in black! ???}
%However, as shown in Figure~\ref{fig:time}c, the Profile List-based methods involve a lower initialization time, which enables them to perform better than the baseline since the early stages of the process.
%For instance, \textsf{CEP-pList} in Figure~\ref{fig:time}b reaches a higher level of recall than \textsf{PSN} only for recall ${>}$ 20\%. {\bf ??? you say that they are better than the baseline at the very beginning, but then you say that they are better only after 20\%; this is confusing! rewrite your argument ???}

%{\color{red}
%The results match our intuition: trading a slightly higher initialization time (w.r.t. the baseline) for a significantly better comparison order is affordable and pays off.
%that the more expensive the matching function is
%}


Hence, the results suggest that the Profile List-based methods are suited for \textsf{ER} tasks involving cheap matching functions, and with very limited time budget.
In particular, considering the results w.r.t. recall progressiveness,
% of Section \ref{sec:recall}, 
the best choice for this scenario become \textsf{LS-PSN}, which involves the lowest overhead.
In all other scenarios, 
%\textsf{BG}-methods 
the Blocking Graph-based methods are the best performers. 
More specifically, \textsf{CEP-pList} achieves the best performance both in terms of recall progressiveness (refer to Figure~\ref{fig:auc}) and execution time (refer to Figure~\ref{fig:time}).

\subsection{Progressiveness on Structured Data}

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=1.0\textwidth]{images/exp/small_50}
	%\vspace{-13pt}
	\caption{Recall progressiveness on
	\textsf{structured} datasets.}
	%\vspace{-8pt}
	\label{fig:small}
\end{figure*} 

\begin{figure}[t!]\centering
	\includegraphics[width=0.49\textwidth]{images/exp/auc_small}
	%\includegraphics[width=0.47\textwidth]{images/exp/auc_large_50}
	\caption{AUC.}
	\label{fig:auc_small}
\end{figure}

%Overall, the best performing method appear to be \textsf{CEP-pList}: in (Figure \ref{fig:time}:a) it outperforms all the other methods when employed with the expensive matching function; and in (Figure \ref{fig:time}b) its performance with the cheap matching function is 

% \note{Add something more here.}

%\vspace{4pt}
%\noindent
%\textbf{Discussion.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DISCUSSION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Giovanni:
% the following comparison with SA-PSN is in part already
% explained at the beginning of Section 5.1.
% However, I added the RED text adapting some of the text below
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Compared to \textsf{SA-PSN}, \textsf{LS-PSN} has higher space requirements, due to $PI$ and the Comparison List. Yet, \textsf{LS-PSN} is more flexible than \textsf{SA-PSN}, as its functionality is configured by the weighting scheme.  
%Combining it with its data structures, \textsf{LS-PSN} yields a better execution order and saves more unnecessary comparisons than \textsf{SA-PSN}.

%Compared to \textsf{SA-PSN}, \textsf{GS-PSN} can achieve higher effectiveness, due to its configuration parameters: $w_{max}$ and the weighting scheme.
%On the downside, its space complexity and initialization time are higher to a significant extent.
%Yet, its emission time is the same as \textsf{SA-PSN}, $O(1)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Giovanni:
% I moved the comparison between GS/LS-PSN is described (5.1).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Compared to \textsf{LS-PSN}, \textsf{GS-PSN} introduces one more configuration parameter, namely $w_{max}$ ($w_{min}$ is set to 1, as in all algorithms that are based on Sorted Neighborhood).
% \textsf{SA-PSN} and \textsf{LS-PSN}. 
%Due to $w_{max}$, \textsf{GS-PSN} trades an initialization phase of higher time and space complexity than \textsf{LS-PSN} for the minimum possible computational cost in the emission phase, $O(1)$. 
%\textsf{GS-PSN} also eliminates all repeated comparisons, gathering in advance all comparisons associated with the window sizes it considers.
%In contrast, \textsf{LS-PSN} is likely to emit the same comparison for two or more different window sizes, as it lacks a mechanism for remembering past emissions.
%Finally, \textsf{GS-PSN} takes into account more co-occurrence patterns when determining comparison weights. 
%In this way, it may result in more accurate estimations than \textsf{LS-PSN} for the likelihood of every comparison to contain duplicates.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Giovanni:
% We do not mention Batch CEP/CNP in any experiment
% If something is needed, I would add it when R-CEP and NC-CEP are described.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%
% Batch CEP vs. R-CEP
%%%%%%%%%%%%%%%%%%
%Compared to \textsf{Batch CEP}, \textsf{R-CEP} involves a higher initialization time and a higher space complexity, as it stores more comparisons in memory.
%It has constant emission time complexity in most of the cases, but raises to the same cost as the initialization time every $K_{max}$ comparisons, i.e., with a frequency that depends on the available memory resources.

%%%%%%%%%%%%%%%%%%
% Batch CEP vs. R-CEP
%%%%%%%%%%%%%%%%%%
%Compared to \textsf{Batch CEP}, we observe that  \textsf{NC-CEP} produces twice as many comparisons, since the same edge may be retained two distinct nodes, but numerous experiments have proven that these correspond to affordable memory requirements \cite{DBLP:conf/edbt/0001PPK16}.
%Most importantly, the recall of \textsf{CNP} (and thus of \textsf{NC-CEP}) is consistently higher than that of \textsf{CEP} to a significant extent \cite{DBLP:journals/tkde/PapadakisKPN14,DBLP:conf/edbt/0001PPK16}.
%This is because the former operates on the local level of individual profiles, while the latter involves a global scope, selecting the best comparisons  across the entire block collection. As a result, \textsf{CEP} ends up retaining no comparison for many profiles that have a duplicate, but are connected with relatively low weights with all co-occurring profiles.




==> section/notation.tex <==
\section{Notation Summary}
\label{sec:notation}

Table \ref{table:notation} summarizes the notation and the metrics employed throughout the paper.

\input{tables/notation}

==> section/taxonomy.tex <==
\section{Taxonomy of Progressive Methods}
{\color{red}

??? TO UPDATE (add [8], i.e., paper ICDE 2017 about progressive ER on MapReduce, which is similar to our na\"ive SA-PSAB) ???

}
\begin{figure}[t!]
\color{blue}
\centering
	\includegraphics[width=0.49\textwidth]{images/taxonomy}
	%\vspace{-12pt}
	\caption{
	Overview of all discussed methods.
	$A {\rightarrow} B$ means that method $B$ builds on method $A$ in order to offer a new functionality.
	}
	\label{fig:taxonomy}
	\vspace{-15pt}
\end{figure}

With respect to the granularity of their functionality, progressive methods are
classified into three main categories, which are called hint types in
\cite{DBLP:journals/tkde/WhangMG13}:
%Comparison-based, Block-based, and Entity-based.
% \noindent

\begin{enumerate}
%\emph{(1)}
\item \textit{Comparison-based methods} provide a list of profile pairs
(i.e., comparisons) that are sorted in descending order of matching likelihood
(from the highest to the lowest one). Then, in the emission phase, profile pairs
are emitted following that ordered list. This category is a generalization of
the category \textit{``sorted list of record pairs''}
\cite{DBLP:journals/tkde/WhangMG13} and includes the methods \textsf{PSN
\cite{DBLP:journals/tkde/PapenbrockHN15, DBLP:journals/tkde/WhangMG13}}, \textsf{SA-PSN}, \textsf{LS-PSN}, and \textsf{GS-PSN}.
% \noindent

%\emph{(2)}

\item \textit{Block-based methods} produce a list of blocks that are sorted in
descending order of the likelihood that they include duplicates among their
profiles.
In the emission phase, all the comparisons for each block are generated,
one block at a time, following that ordered list;~all comparisons in the same
block have the same matching likelihood. This is a generalization of the
category \textit{``hierarchy of record partitions''}
\cite{DBLP:journals/tkde/WhangMG13} and includes the homonymous method
\textsf{HRP} \cite{DBLP:journals/tkde/WhangMG13} together with \textsf{SA-PSAB}.

%\emph{(3)}
\item\textit{Profile-based methods} provide a list of profiles that are sorted
in descending order of duplication likelihood. Then, in the emission phase, all
comparisons of every entity are generated, one entity at a time,
following that ordered list. This category is a generalization of the category
\textit{``ordered list of records''} \cite{DBLP:journals/tkde/WhangMG13} and
includes the homonymous method \textsf{OLR} \cite{DBLP:journals/tkde/WhangMG13}.

\end{enumerate}

We illustrate this categorization in Figure \ref{fig:taxonomy}, where every
column corresponds to a different type of granularity. Note that we have also
added a fourth column, which corresponds to the category of \textit{hybrid
methods}. These are methods that combine characteristics from two or all of the
previous categories. For example, it includes \textsf{PBS}, which involves both
block- and comparison-based characteristics, as well as \textsf{PPS}, which
combines comparison-based characteristics with profile-based ones.

Note that Figure \ref{fig:taxonomy} maps all progressive methods discussed
in this work to the corresponding granularity category (horizontal axis). On
the vertical axis, we consider the relation of every method to schema knowledge,
with the topmost part corresponding to batch methods.
% columns classify the methods on the basis of their granularities.
Every arrow from method $A$ to method $B$ means that $B$ extends $A$ in order to
offer a new functionality. For instance, \textsf{PBS} and \textsf{PPS}
are based on the Blocking Graph, which is the core data structure of
Batch Meta-blocking \cite{DBLP:conf/edbt/0001PPK16}.




%These categories correspond to the three leftmost columns of Figure~\ref{fig:methodsOverview}, which also depicts the methods they comprise.


==> section/taxonomy_old.tex <==
\subsection{Taxonomy}
\label{sec:taxonomy}

To facilitate the use and understanding of existing and new methods for
\textsf{Progressive ER}, we introduce a taxonomy that organizes them
according to the following four criteria.

\textbf{Scope.} This criterion pertains to the functionality granularity of a
progressive method, defining four categories:

\emph{(i)} \textit{Comparison-based methods} operate on the level of
pairs of entities (i.e., comparisons), aiming to optimize their execution order.
Basically, they sort all comparisons in decreasing likelihood that they involve a pair of
matching entities: the first position corresponds to the comparison with the
highest likelihood and the last one to the comparison with the lowest
likelihood. Methods of this scope correspond to the category ``\textit{sorted
list of record pairs}'' \cite{DBLP:journals/tkde/WhangMG13}. 

\emph{(ii)} \textit{Block-based methods} operate on the level of groups of
entities (i.e., blocks), trying to determine their optimal processing order. To
this end, they organize the given entities in a hierarchy of blocks, with
every level corresponding to a different granularity: the bottom-most level
contains the smallest blocks, which grow larger as we move to higher levels.
The execution starts from the bottom-most level and moves up to
the top level. Methods of this scope correspond to the category
``\textit{hierarchy of record partitions}'' \cite{DBLP:journals/tkde/WhangMG13}.

\emph{(iii)} \textit{Entity-based methods} operate on the level of individual
entities, determining their optimal processing order: they sort all
entities in decreasing likelihood that they match with another entity, from the
entities with the highest chances to the entity with the lowest ones. Methods of
this scope correspond to the category ``\textit{sorted list of records}'' \cite{DBLP:journals/tkde/WhangMG13}.
  
\emph{(iv)} \textit{Hybrid methods} combine characteristics from at least two
of the above functionality granularities.

The first three categories have already been examined in the literature, while
the last one is new. Apparently, entity-based methods correspond to the  most
fine-grained functionality, while block-based methods involve the most
coarse-grained one. In general, the finer the granularity is, the more
time-consuming is the corresponding functionality.

\textbf{Adaptivity.} This criterion characterizes the nature of the
processing order that is defined by a progressive method. There are two
possible options:

\emph{(i)} \textit{Static methods} are independent of entity matching, 
defining an immutable processing order up front.
  
\emph{(ii)} \textit{Dynamic methods} are integrated with entity matching,
adjusting their processing order on-the-fly. In fact, they assume the
use of an oracle that always decides with 100\% accuracy whether two entities are matching
or not. Based on the new evidence that is offered by the latest identified
matches, they guide the processing to entities that are more likey to match.
However, in the absence of a noise-free entity matching method, their
assumption is unrealistic, yielding an optimistic performance.

{\color{red} I am not sure whether the following is true: Additionally, these
methods are useful only for Dirty ER, where every entity is likely to have multiple duplicates. In other words, they are
incompatible with Clean-Clean ER, where every entity is matching with at most
one other entity.}
%\note{
%For out ``entity level'' PMB, which is a sort of ``hybrid'' comparisons-entity level, the results are in the experiments also for cleaningER.
%Here the idea is that retaining the top-first comparison for each node comes for free while computing the entity weights.
%}

\textbf{Background.} This criterion expresses the relation of 
a progressive method with the background knowledge about the given entity
collection. It defines two types of methods:

\emph{(i)} \textit{Schema-based methods} require domain knowledge in the form
  of schema information that characterizes the noise and discriminativeness
  of every attribute value.
   
\emph{(ii)} \textit{Schema-agnostic methods} are independent of any schema
information and any other domain knowledge. 

\textbf{Configuration.} This criterion defines two types of methods
based on how they fine-tune their internal parameters:

\emph{(i)} \textit{Supervised methods} require a training set for learning
how to rank the items they operate on.

\emph{(ii)} \textit{Unsupervised methods} rank their input items independently
of any training set.

\begin{figure}[ht!]\centering
	\includegraphics[width=0.45\textwidth]{images/taxonomy}
	\vspace{-12pt}
	\caption{An example of an image we could use for organizing our methods into
	a taxonomy.}
	\vspace{-15pt}
	\label{fig:taxonomy}
\end{figure}

{\color{red}\textbf{Performance.} This criterion examines the performance goal
of Progressive Methods with respect to recall. Two options are possible:

\begin{enumerate}
  \item \textit{Exhaustive methods} aim to identify all pairs of duplicates
  (100\% recall).
  \item \textit{Approximate methods} sacrifice recall to a minor extent in order
  to achieve significant gains in efficiency.
\end{enumerate}}

==> tables/notation.tex <==
{\renewcommand{\arraystretch}{1.25}
\begin{table}[t!]
\centering
%\scriptsize
%\small
\begin{tabular}{| r | l |}
\multicolumn{2}{c}{\textsc{Symbols:}}\\
\hline
$p_i$ & an entity profile with id $i$ \\
\hline
$P$ & a set of profiles\\
\hline
$c_{ij}$ & a comparison between profiles $p_i$ and $p_j$\\
\hline
${p_i\equiv p_j}$ & two matching profiles\\
%\hline
%$k_x$& a blocking key\\
\hline
$b_k$ & a block with id $k$ \\
\hline
$|b_k|$ & block size (no. of profiles)\\
\hline
$\|b_k\|$ & block cardinality (no. of comparisons)\\
\hline
$B$ & a block collection\\
\hline
$|B|$ & block collection size (no. of blocks)\\
\hline
$\|B\|$ & block cardinality (total no. of comparisons)\\
%\hline
%$|b_k|$ & no. of profiles in $b_k$\\
%\hline
%$\|b_k\|$ & no. of comparisons entailed by $b_k$\\
%\hline
%$B$, $|B|$, $\|B\|$ & a block collection, its size (no. of blocks), its cardinality (no. of comparisons)\\
%$B$& a block collection\\
%\hline
%$|B|$ & no. of blocks in $B$\\
%\hline
%$\|B\|$ & no. of comparisons entailed by $B$\\
\hline
$B_i$& the set of blocks containing profile $p_i$\\
\hline
% $\kpp$ & {average no. of \textbf{k}eys \textbf{p}er \textbf{p}rofile} \\ 
% \hline
% $\ppb$ & {average no. of \textbf{p}rofile \textbf{p}er \textbf{b}lock} \\
$\bar{|p|}$ & {average no. of keys per profile} \\ 
\hline
$\bar{|b|}$ & {average block size}\\
\hline
\multicolumn{2}{c}{\textsc{Method Acronyms:}}\\
\hline
\textsf{PSN} & Progressive Sorted Neighborhood \\
\hline
\textsf{SA-PSN} & Schema-agnostic \textsf{PSN}\\
\hline
\textsf{LS-PSN} & Local Schema-agnostic \textsf{PSN} \\
\hline
\textsf{GS-PSN} & Global Schema-agnostic \textsf{PSN} \\
\hline
\textsf{RCF} & Relative Co-occurrence Frequency \\
\hline
\textsf{PBS} & Progressive Block Scheduling \\
\hline
\textsf{PPS} & Progressive Profile Scheduling \\
\hline
\textsf{ARCS} & Aggregate Reciprocal Comparisons Scheme \\
\hline
\textsf{SAB} & Suffix Arrays Blocking \\
\hline
\textsf{SA-PSAB} & Schema-agnostic \textsf{SAB}\\
\hline
\textsf{HRP} & Hierarchy of Record Partitions \\
\hline
\textsf{OLR} & Ordered List of Records \\
\hline
\multicolumn{2}{c}{\textsc{Metrics:}}\\
\hline
$\mathcal{D}_P$ & {no. of duplicates in $P$}\\
\hline
$\mathcal{D}_m$ & {no. of duplicates emitted}\\
\hline
recall & {$|\mathcal{D}_m|/|\mathcal{D}_P|$}\\
\hline
$ec$ & {no. emitted comparisons}\\
\hline
$ec^*$&{$ec/|\mathcal{D}_P|$}\\
\hline
$AUC_m$ & \makecell[l]{area under the curve of the recall\\ of a method $m$ plotted in function of $ec*$}\\
\hline
$AUC_m^*$ & \makecell[l]{$AUC_m$ normalized by the AUC of the ideal method}\\
\hline

\end{tabular}
\vspace{5pt}
\caption{Notation summary.}
\vspace{-18pt}
\label{table:notation}
\end{table}
}
